Nonparametric Stochastic Compositional Gradient Descent for Q-Learning in Continuous Markov Decision Problems

We consider Markov Decision Problems defined over continuous state and action spaces, where an autonomous agent seeks to learn a map from its states to actions so as to maximize its long-term discounted accumulation of rewards. We address this problem by considering Bellman's optimality equation defined over action-value functions, which we reformulate into a nested non-convex stochastic optimization problem defined over a Reproducing Kernel Hilbert Space (RKHS). We develop a functional generalization of stochastic quasi-gradient method to solve it, which, owing to the structure of the RKHS, admits a parameterization in terms of scalar weights and past state-action pairs which grows proportionately with the algorithm iteration index. To ameliorate this complexity explosion, we apply Kernel Orthogonal Matching Pursuit to the sequence of kernel weights and dictionaries, which yields a controllable error in the descent direction of the underlying optimization method. We prove that the resulting algorithm, called KQ-Learning, converges with probability 1 to a stationary point of this problem, yielding a fixed point of the Bellman optimality operator under the hypothesis that it belongs to the RKHS. Under constant learning rates, we further obtain convergence to a small Bellman error that depends on the chosen learning rates. Numerical evaluation on the Continuous Mountain Car and Inverted Pendulum tasks yields convergent parsimonious learned action-value functions, policies that are competitive with the state of the art, and exhibit reliable, reproducible learning behavior.

==> proof.tex <==
%!TEX root = main.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%     S  E  C  T  I  O  N    %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \section{Convergence Analysis}\label{sec:convergence}
 
In this section, we shift focus to the task of establishing that the sequence of action-value function estimates generated by Algorithm \ref{qlearning} actually yield a locally optimal solution to the Bellman optimality equation, which, given intrinsic the non-convexity of the problem setting, is the best one may hope for in general through use of numerical stochastic optimization methods. Our analysis extends the ideas of coupled supermartingales in reproducing kernel Hilbert spaces \cite{pkgtd}, which have been used to establish convergent policy evaluation approaches in infinite MDPs (a convex problem), to non-convex settings, and further generalizes the non-convex vector-valued setting of \cite{wang2017stochastic}. 

Before proceeding with the details of the technical setting, we introduce a few definitions which simplify derivations greatly. In particular, for further reference, we use \eqref{eq:actargmax} to define   $\mathbf{a}_t' = \argmax_{\mathbf{a}_t'} Q_t(\mathbf{s}_t',\mathbf{a}_t')$, the instantaneous maximizer of the action-value function and defines the direction of the gradient.  We also define the functional stochastic quasi-gradient of the regularized objective
%
\begin{align} \label{eq:unprojectedgradproof}
%
\hat{\nabla}_Q & J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') =  \nonumber \\ & (\gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) 
-\kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot))z_{t+1} + \lambda Q_t
%
\end{align}
%
 and its sparse-subspace projected variant as
 %
 \begin{align} \label{eq:projectedgradproof}
 %
 & \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') = \nonumber \\ & \!\! (Q_t \!\! - \!\! \mathcal{P}_{\ccalH_{D_{t+1}}} \!\! \lbrack Q_t - {\alpha}_t \!\! \hat{\nabla \!}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') \rbrack ) \! / \! \alpha_t
 %
 \end{align}
 %
 Note that the update may be rewritten as a stochastic projected quasi-gradient step rather than a stochastic quasi-gradient step followed by a set projection, i.e.,
 %
 \begin{equation} \label{eq:qprojectedupdateproof}
 %
 Q_{t+1} = Q_t - {\alpha}_t  \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t')
 %
 \end{equation}
 %
With these definitions, we may state our main assumptions required to establish convergence of Algorithm \ref{qlearning}.\vspace{-5mm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%A  S  S  U  M  P  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:compact}
The state space  $\mathcal{S} \subset \mathbb{R}^p$ and action space $\mathcal{A} \subset \mathbb{R}^q$ are compact, and the reproducing kernel map may be bounded as
%
\begin{equation} \label{eq:boundedkernelproof}
%
\sup_{\mathbf{s} \in \mathcal{S}, \mathbf{a} \in \mathcal{A}} \sqrt{\kappa((\mathbf{s},\mathbf{a}),(\mathbf{s},\mathbf{a}))} = K < \infty
%
\end{equation}
%
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%A  S  S  U  M  P  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:mean_variance_delta}
 The temporal action difference $\delta$ and auxiliary sequence $z$ satisfy the zero-mean, finite conditional variance, and Lipschitz continuity conditions, respectively,
%
\begin{equation} \label{eq:mean_variance_delta}
%
\!\!\! \mathbb{E} \lbrack \delta \! \mid \! \mathbf{s},\mathbf{a} \rbrack = \bar{\delta} \; , \ 
 \mathbb{E} \lbrack (\delta \! - \! \bar{\delta})^2\rbrack \! \leq \! {\sigma}_{\delta}^2 \; ,\
 \mathbb{E} \lbrack z^2 \! \mid \! \mathbf{s}, \mathbf{a} \rbrack \! \leq \! G_{\delta}^2  
%
\end{equation}
%
where $\sigma_{\delta}$ and $G_{\delta}$ are positive scalars, and $\bar{\delta} = \mathbb{E} \lbrace \delta \mid \mathbf{s}, \mathbf{a} \rbrace$ is defined as the expected value of the temporal action difference conditioned on the state $\bbs$ and action $\mathbf{a}$.
\end{assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%A  S  S  U  M  P  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:mean_variance_q}The functional gradient of the temporal action difference is an unbiased estimate for $\nabla_Q J(Q)$ and the difference of the reproducing kernels expression has finite conditional variance:
%
\begin{equation} \label{eq:finitevariance1proof}
%
\mathbb{E} \lbrack (\gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) - \kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot))\delta \rbrack = \nabla_Q J(Q)
%
\end{equation}
%
\begin{equation} \label{eq:finitevariance2proof}
%
\mathbb{E} \lbrace \| \gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) - \kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot) \|^2_{\ccalH}|\mathcal{F}_t\rbrace \leq G_Q^2
%
\end{equation}
Moreover, the projected stochastic quasi-gradient of the objective has finite second conditional moment as 
%
\begin{equation} \label{eq:finitemomentproof}
%
\mathbb{E} \lbrace \|  \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') \|^2_{\ccalH}|\mathcal{F}_t\rbrace \leq {\sigma}_Q^2
%
\end{equation}
%
and the temporal action difference is Lipschitz continuous with respect to the action-value function Q. Moreover, for any two distinct $\delta$ and $\bar{\delta}$, we have 
%
\begin{equation} \label{eq:deltaqproof}
%
\|\delta - \bar{\delta}\| \leq L_Q \| Q - \tilde{Q} \|_{\ccalH}
%
\end{equation}
%
with $Q$, $\tilde{Q} \in \ccalH$ distinct $Q$-functions; $L_Q > 0$ is a scalar.
\end{assumption}

Assumption \ref{as:compact} regarding the compactness of the state and action spaces of the MDP holds for most application settings and limits the radius of the set from which the MDP trajectory is sampled. The mean and variance properties of the temporal difference stated in Assumption \ref{as:mean_variance_delta} are necessary to bound the error in the descent direction associated with the stochastic sub-sampling and are required to establish convergence of stochastic methods. Assumption \ref{as:mean_variance_q} is similar to Assumption \ref{as:mean_variance_delta}, but instead of establishing bounds on the stochastic approximation error of the temporal difference, limits stochastic error variance in the RKHS. Moreover, \eqref{eq:deltaqproof} is justified since the maximum of a continuous function is Lipschitz in the infinity norm, which can be related to the Hilbert norm through a constant factor. These are natural extensions of the conditions needed for vector-valued stochastic compositional gradient methods.

The compactness of $\mathcal{S}$ and $\mathcal{A}$ (Assumption \ref{as:compact}) implies that $\ccalH$ is a compact function space, which together with the closedness of Hilbert subspaces ${\ccalH}_{D_t}$, mean $Q_t$ is contained within compact sets for all $t$ due to the use of set projections in \eqref{eq:proj_fsqg}, meaning
 %
 \begin{equation} \label{eq:compactnessproof}
 %
 \|Q_t\|_{\ccalH} \leq D \text{ for all } t \; ,
 %
 \end{equation}
 %
where $D > 0$ is some positive constant.  

Next, we turn to establishing some technical results which are necessary precursors to the proofs of the main stability results. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%P  R  O  P  O  S  I  T  I  O  N  %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proposition}\label{prop_proj_grad_err} Given independent identical realizations $(\mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t')$ of the random triple $(\mathbf{s},\mathbf{a},\mathbf{s}')$, the difference between the projected stochastic functional quasi-gradient and the stochastic functional quasi-gradient of the instantaneous cost is bounded for all $t$ as
%
\begin{align} \label{eq:prop1proof}
%
\!\!\!\!   \|\! \tilde{\nabla}_{\!Q} J(\!Q_t, \! z_{t\!+\!1} \!;  \mathbf{s}_t\!, \! \mathbf{a}_t\!, \! \mathbf{s}_t'\!)\! -\!\!  \hat{\nabla}_{\!Q} J(\!Q_t, \! z_{t\!+\!1} \!;  \mathbf{s}_t\!, \! \mathbf{a}_t\!, \!\mathbf{s}_t'\!) \!\|_{\ccalH} \!\!\leq \!\!\! \frac{\epsilon_t}{\alpha_t}
%
\end{align}
%
Where $\alpha_t > 0$ denotes the algorithm step size and $\epsilon_t > 0$ is the compression budget parameter of the KOMP algorithm. 
\end{proposition}

\begin{myproof}
As in Proposition 1 of \cite{pkgtd}, Consider the square-Hilbert norm difference of $\tilde{\nabla}_Q J(Q_t, z_{t+1};   \mathbf{s}_t,\mathbf{a}_t, \mathbf{s}_t')$ and $\hat{\nabla}_Q  J(Q_t, z_{t+1};   \mathbf{s}_t,\mathbf{a}_t, \mathbf{s}_t')$ defined by \eqref{eq:unprojectedgradproof} and \eqref{eq:projectedgradproof}
%
\begin{align} \label{eq:prop1aproof}
%
\| \tilde{\nabla}_Q & J(Q_t, z_{t+1};   \mathbf{s}_t,\mathbf{a}_t, \mathbf{s}_t') - \hat{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') \|_{\ccalH} =
\nonumber \\  
 \| & (Q_t -  \mathcal{P}_{\ccalH_{\mathbf{D}_{t+1}}}  \lbrack Q_t - \alpha_t \hat{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t, \mathbf{a}_t, \mathbf{s}'_t) \rbrack  )/\alpha_t 
\nonumber \\  
&  -   \hat{\nabla}_Q J(Q_t, z_{t+1}\!; \mathbf{s}_t, \mathbf{a}_t, \mathbf{s}'_t) \|_\ccalH^2
%
\end{align}
%
Multiply and divide $\hat{\nabla}_Q  J(Q_t, z_{t+1};   \mathbf{s}_t,\mathbf{a}_t, \mathbf{s}_t')$ by $\alpha_t$ and reorder terms to write
%
\begin{align} \label{eq:prop1bproof}
%  
 \| & \frac{(Q_t -  \alpha_t \hat{\nabla}_Q J(Q_t, z_{t+1}\!; \mathbf{s}_t, \mathbf{a}_t, \mathbf{s}'_t)  )}{\alpha_t} 
\nonumber \\ &
- \frac{(\mathcal{P}_{\ccalH_{\mathbf{D}_{t+1}}}  \lbrack Q_t - \alpha_t \hat{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t, \mathbf{a}_t, \mathbf{s}'_t) \rbrack  )}{\alpha_t} 
\|_\ccalH^2   
\nonumber \\ 
= & \frac{1}{\alpha_t^2} \| (Q_t -  \alpha_t \hat{\nabla}_Q J(Q_t, z_{t+1}\!; \mathbf{s}_t, \mathbf{a}_t, \mathbf{s}'_t)  )
\nonumber \\ &
- (\mathcal{P}_{\ccalH_{\mathbf{D}_{t+1}}}  \lbrack Q_t - \alpha_t \hat{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t, \mathbf{a}_t, \mathbf{s}'_t) \rbrack  ) \|_\ccalH^2
\nonumber \\ 
= & \frac{1}{\alpha_t^2} \| \tilde{Q}_{t+1} - Q_{t+1} \|_\ccalH^2 \leq \frac{\epsilon_t^2}{\alpha_t^2}
%
\end{align}
%
where we have pulled the nonnegative scalar $\alpha_t$ outside of the norm on the second line and substituted the definition of $\tilde{Q}_{t+1}$ and $Q_{t+1}$. We also apply the KOMP residual stopping criterion from Algorithm 2, $\| \tilde{Q}_{t+1} - Q_{t+1} \| \leq \epsilon_t$ to yield \eqref{eq:prop1proof}.
\end{myproof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%L  E  M  M  A  %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{main_lemma} Denote the filtration $\mathcal{F}_t$ as the time-dependent sigma-algebra containing the algorithm history $( \lbrace Q_u, z_u\rbrace_{u=0}^t   \cup \lbrace \mathbf{s}_u, \mathbf{a}_u, \mathbf{s}_u' \rbrace_{u=0}^{t-1}) \subset \mathcal{F}_t$. Let Assumptions \ref{as:compact}-\ref{as:mean_variance_q} hold true and consider the sequence of iterates defined by Algorithm \ref{qlearning}. Then:
\begin{enumerate}[i.]
%
\item The conditional expectation of the Hilbert-norm difference  of action-value functions at the next and current iteration satisfies the relationship \label{main_lemma_1}
%
\begin{equation} \label{eq:lemma1iproof}
%
 \! \! \mathbb{E} \lbrack \| Q_{t+1} \!- \!Q_t \|^2_{\ccalH}\!  \! \mid\!\! \mathcal{F}_t \rbrack \!\! \leq \! 2 \alpha^2_t \!(\!G_{\delta}^2G_Q^2 \!+ \! \! \lambda \! D^2 \!) \! + \! 2  \epsilon_t^2
%
\end{equation}
%
\item The auxiliary sequence $z_t$ with respect to the conditional expectation of the temporal action difference $\bar{\delta}_t$ (defined in Assumption \ref{as:mean_variance_delta}) satisfies \label{main_lemma_2}
%
\begin{align} \label{eq:lemma1iiproof}
%
\!\mathbb{E} \lbrack  (z_{t+1} -  \bar{\delta_t})^2 \mid \! \mathcal{F}_t\!  \rbrack & \leq (1-\beta_t)(z_t - \bar{\delta}_{t-1})^2  \\ 
&\quad + \frac{L_Q}{\beta_t} \|Q_t \!-\! Q_{t-1}\|^2_\ccalH + 2 \beta_t^2 \sigma_{\delta}^2\nonumber
%
\end{align}
%
\item Algorithm \ref{qlearning} generates a sequence of Q-functions that satisfy the stochastic descent property with respect to the Bellman error $J(Q)$ [cf. \eqref{eq:lossprob}]: \label{main_lemma_3}
%
\begin{align} \label{eq:lemma1iiiproof}
%
\mathbb{E}[J(\!Q_{t+1}\!)\given\ccalF_t] &\leq   J(\!Q_t\!)
- \alpha_t \!\!\left(\!\!1\! -\! \frac{\alpha_t G_{Q}^2 }{ \beta_t}\!\!\right) \|\nabla_Q J(Q)\|^2\! \!
\nonumber \\ 
&\quad+\!  \frac{\beta_t}{2} \mathbb{E} \lbrack ( \bar{\delta_t} - z_{t+1} )^2 \mid \mathcal{F}_t \rbrack+\frac{L_Q \sigma_Q^2 \alpha_t^2}{2} \nonumber \\
&\quad + \eps_t \|\nabla_Q J(Q_t) \|_{\ccalH} \; ,
%
\end{align}
%
\end{enumerate}
%
\end{lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% P  R  O  O  F  %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{myproof} \textit{Lemma \ref{main_lemma}\eqref{main_lemma_1} }
Consider the Hilbert-norm difference of action-value functions at the next and current iteration and use the definition of $Q_{t+1}$
%
\begin{equation} \label{eq:aproof}
%
\!\! \|Q_{t+1} \!\! - \!\! Q_t \! \|_\ccalH^2 \!\! = \!\! \alpha_t^2 \| \!\tilde{\nabla}_Q J(Q_t, z_{t+1}\!;\! (\mathbf{s}_t,\mathbf{a}_t),(\mathbf{s}_t'\!,\mathbf{a}_t'\!) \|_\ccalH^2 \!
%
\end{equation}
%
We add and subtract the functional stochastic quasi-gradient $\hat{\nabla}_Q J(Q_t, z_{t+1}; (\mathbf{s}_t,\mathbf{a}_t),(\mathbf{s}_t',\mathbf{a}_t')$ from \eqref{eq:aproof} and apply the triangle inequality $(a+b)^2 \leq 2a^2 + 2b^2$ which holds for any $a,b>0$.
%
\begin{align} \label{eq:bproof}
%
\!\!\|Q_{t+1} \! - \! Q_t\|_\ccalH^2  
&\leq 2 \alpha_t^2 \|\hat{\nabla}_Q J(Q_t, z_{t+1}; (\mathbf{s}_t,\mathbf{a}_t),(\mathbf{s}_t',\mathbf{a}_t') \|_\ccalH^2 
\nonumber \\
&\quad + \! 2 \alpha_t^2  \|\hat{\nabla}_Q J(Q_t, z_{t+1}; (\mathbf{s}_t,\mathbf{a}_t),(\mathbf{s}_t',\mathbf{a}_t')  
\nonumber \\ 
&\quad  - \!\tilde{\nabla}_Q J(Q_t, z_{t+1}\!; (\mathbf{s}_t\!,\mathbf{a}_t\!)\!,\!(\mathbf{s}_t'\!,\mathbf{a}_t') \|_\ccalH^2
%
\end{align}
%
 Now, we may apply Proposition 1 to the second term. Doing so and computing the expectation conditional on the filtration $\mathcal{F}_t$ yields
 %
 \begin{align} \label{eq:cproof}
 %
 \!\!   \mathbb{E}  &\lbrack \|Q_{t+1} - Q_t\|_\ccalH^2 \rbrack \mid \mathcal{F} \rbrack  
 \\
 &=  2 \alpha_t^2 \mathbb{E} \lbrack \|\hat{\nabla}_Q J(Q_t, z_{t+1}; (\mathbf{s}_t,\mathbf{a}_t),(\mathbf{s}_t',\mathbf{a}_t') \|_\ccalH^2 \mid \mathcal{F}_t \rbrack \! + \! 2 \epsilon_t^2\nonumber
 %
 \end{align}
 %
Using the Cauchy-Schwarz inequality together with the Law of Total Expectation and the definition of the functional stochastic quasi-gradient to upper estimate the first term on the right-hand side of \eqref{eq:cproof} as
%
\begin{align} \label{eq:dproof}
%
 \mathbb{E}  \lbrack  \| Q_{t+1}  &-  Q_t\|^2_\ccalH \mid \mathcal{F}_t \rbrack  
 \\
& \leq  2 \alpha_t^2 \mathbb{E} \lbrace \| \gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) - \! \kappa((\mathbf{s}_t,\mathbf{a}_t),\!\cdot\!) \|_\ccalH^2 
\nonumber \\
&\quad\times \mathbb{E} \lbrack z_{t+1}^2 \! \mid \mathbf{s}_t, \! a_t \rbrack \mid \mathcal{F}_t \! \rbrace 
\!\! + \!\! 2 \alpha_t^2 \!\! \lambda \|Q_t\|_\ccalH^2 \! \!\! + \!\! 2 \epsilon_t^2
\nonumber
%
\end{align}
%
Now, use the fact that $z_{t+1}$ has a finite second conditional moment [cf. \eqref{eq:mean_variance_delta}], yielding
%
\begin {align}  \label{eq:eproof}
%
\mathbb{E}  \lbrack & \|Q_{t+1} -  Q_t\|^2_\ccalH \mid \mathcal{F}_t \rbrack
\nonumber \\
& \quad\leq  2 \alpha_t^2 G_\delta^2 \mathbb{E} \lbrack \| \gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) 
- \kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot) \|_\ccalH^2  \mid \mathcal{F}_t \rbrack 
\nonumber \\
& \qquad+ 2 \alpha_t^2 \lambda \|Q_t\|_\ccalH^2 + 2 \epsilon_t^2
%
\end{align}
%
From here, we may use the fact that the functional gradient of the temporal action-difference $\gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) - \kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot)$ has a finite second conditional moment \eqref{eq:mean_variance_delta} and that the $Q$ function sequence is bounded \eqref{eq:compactnessproof} to write:
%
\begin{equation} \label{eq:fproof}
%
\mathbb{E} \lbrack \|Q_{t+1} \!\! - \! Q_t\|^2_\ccalH \mid \mathcal{F}_t \rbrack \leq 2 \alpha_t^2 (G_\delta^2 G_V^2  \! +  \! \! \lambda^2 D^2) \! + \! 2 \epsilon_t^2
%
\end{equation}
%
which is as stated in Lemma \ref{main_lemma}\eqref{main_lemma_1}.
\end{myproof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% P  R  O  O  F  %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{myproof} \textit{Lemma \ref{main_lemma}\eqref{main_lemma_2} }
Begin by defining the scalar quantity $e_t$ as the difference of mean temporal-action differences scaled by the forgetting factor $\beta_t$, i.e. $e_t = (1-\beta_t)(\bar{\delta_t} - \bar{\delta}_{t-1})$. Then, we consider the difference of the evolution of the auxiliary variable  $z_{t+1}$ with respect to the conditional mean temporal action difference $\bar{\delta}_t$, plus the difference of the mean temporal differences:
%
\begin{align} \label{eq:gproof}
%
z_{t+1} - \bar{\delta}_t + e_t =  & (1-\beta_t)z_t + \beta_t\delta_t - \lbrack(1-\beta_t)\bar{\delta_t} + \beta_t \bar{\delta_t} \rbrack
\nonumber \\ 
& + (1-\beta_t)(\bar{\delta_t} - \bar{\delta}_{t-1}) 
%
\end{align}
%
where we make use of the definition of $z_{t+1}$, the fact that $\bar{\delta}_t = \lbrace (1-\beta_t)\bar{\delta}_t + \beta_t \bar{\delta}_t \rbrace$ and the definition of $e_t$ on the right-hand side of \eqref{eq:gproof}. Observe that the result then simplifies to $z_{t+1} - \bar{\delta}_t + e_t=(1-\beta_t)z_t +  \beta_t(\bar{\delta_t} - \bar{\delta}_{t-1}) $ by grouping like terms and canceling the redundant $\bar{\delta}_t$. Squaring \eqref{eq:gproof}, using this simplification, yields
%
\begin{align} \label{eq:hproof}
%
(z_{t+1} - &\bar{\delta}_t + e_t)^2 
\nonumber \\
&=  (1-\beta_t)^2(z_t - \bar{\delta}_{t-1})^2 
+ \beta_t^2(\delta_t - \bar{\delta}_t)^2 
\nonumber \\
&\quad+ 2(1-\beta_t)\beta_t(z_t-\bar{\delta}_{t-1})(\delta_t - \bar{\delta_t}) 
%
\end{align}
%
Now, let's compute the expectation conditioned on the algorithm history $\mathcal{F}_t$ to write
%
\begin{align} \label{eq:iproof}
%
\mathbb{E}\lbrack(z_{t+1} & - \bar{\delta}_t + e_t)^2 \mid \mathcal{F}_t\rbrack 
\nonumber \\
= & (1-\beta_t)^2(z_t - \bar{\delta}_{t-1})^2 + \beta_t^2  \mathbb{E}  \lbrack(\delta_t - \bar{\delta}_t)^2 \mid \mathcal{F}_t\rbrack  
\nonumber \\  
 &+ 2(1-\beta_t)\beta_t(z_t-\bar{\delta}_{t-1})\mathbb{E}\lbrack(\delta_t - \bar{\delta_t}) \mid \mathcal{F}_t\rbrack
%
\end{align}
%
We apply the assumption that the temporal action difference $\delta_t$ is an unbiased estimator for its conditional mean $\bar{\delta}_t$ with finite variance (Assumption \ref{as:mean_variance_delta}) to write
%
\begin{equation} \label{eq:kproof}
%
\!\! \mathbb{E} \lbrack (z_{t+1} \!\! - \! \bar{\delta}_t \! +  \! e_t) \! \given  \! \ccalF_t \rbrack \! = \! (1 \!- \! \beta_t)^2 (z_t \! - \! \bar{\delta}_{t-1})^2 \! + \! \beta_t^2 \! \sigma_\delta^2
%
\end{equation}
%
We obtain an upper estimate on the conditional mean square of $z_{t+1} - \bar{\delta}_t$ by using the inequality $\| a + b \|^2 \leq (1+\rho) \| a \|^2 + (1+1 \rho) \| b \|^2$ which holds for any $\rho > 0$: set $a=z_{t+1} - \bar{\delta}_t + e_t$, $b = -e_t$, $\rho = \beta_t$ to write
\begin{equation} \label{eq:lproof}
%
\!\!\!\!\!(z_{t+1} \! - \! \bar{\delta}_t)^2 \! \leq \! (1+\beta_t)(z_{t+1} \! - \! \bar{\delta}_t \! + \! e_t)^2 \! + \! \left(1 \! + \! \frac{1}{\beta_t}\right) e_t^2
%
\end{equation}
%
Observe that \eqref{eq:lproof} provides an upper-estimate of the square sub-optimality $(z_{t+1} - \bar{\delta}_t)^2$ in terms of the squared error sequence $(z_{t+1} \! - \! \bar{\delta}_t \! + \! e_t)^2 $. Therefore, we can compute the expectation of \eqref{eq:lproof} conditional on $\ccalF_t$ and substitute \eqref{eq:kproof} for the terms involving the error sequence $(z_{t+1} \! - \! \bar{\delta}_t \! + \! e_t)^2 $, which results in gaining a factor of $(1+\beta_t)$ on the right-hand side. Collecting terms then yields
%
\begin{align} \label{eq:mproof}
%
&\mathbb{E}  \lbrack (z_{t+1} - \bar{\delta}_t)^2 \mid \mathcal{F}_t \rbrack  
\\
&  = (1+\beta_t)  \lbrack (1-\beta_t)^2(z_t\! -\! \bar{\delta}_{t-1})^2 + \beta_t^2\sigma_\delta^2 \rbrack + \left(\!\!\frac{1+\beta_t}{\beta_t}\!\!\right) e_t^2 
\nonumber
%
\end{align} 
%
Using the fact that $(1-\beta_t^2)(1-\beta_t) \leq (1-\beta_t)$ for the first term and $(1-\beta_t)\beta_t^2 \leq 2 \beta_t^2$ for the second to simplify
%
\begin{align} \label{eq:nproof}
%
\mathbb{E} \lbrack (z_{t+1} - \bar{\delta}_t)^2 \mid \mathcal{F}_t \rbrack  
=  & (1-\beta_t)(z_t - \bar{\delta}_{t-1})^2 + 2\beta_t^2\sigma_\delta^2 
\nonumber \\ & 
\quad + \left(\frac{1+\beta_t}{\beta_t}\right) e_t^2
%
\end{align}
%
We can bound the term involving $e_t$, which represents the difference of mean temporal differences. By definition, we have $|e_t| = (1- \beta_t)|(\bar{\delta}_t  -  \bar{\delta}_{t-1})|$:
%
\begin{equation} \label{eq:oproof}
%
(1\!-\! \beta_t)|(\bar{\delta}_t \! - \! \bar{\delta}_{t-1})| \! \leq \! (1 \!- \! \beta_t) L_Q \| Q_t \! - \! Q_{t-1} \! \|_\ccalH \; ,
%
\end{equation}
%
where we apply the Lipschitz continuity of the temporal difference with respect to the action-value function [cf. \eqref{eq:deltaqproof}]. Substitute the right-hand side of \eqref{eq:oproof} and simplify the expression in the last term as $(1-\beta_t^2) / \beta_t \leq 1/\beta_t$ to conclude \eqref{eq:lemma1iiiproof}.
 \end{myproof} 
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% P  R  O  O  F  %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{myproof} \textit{Lemma \ref{main_lemma}\eqref{main_lemma_3} }
Following the proof of Theorem 4 of \cite{wang2017stochastic}, we begin by considering the Taylor expansion of $J(Q)$ and applying the fact that it has Lipschitz continuous functional gradients to upper-bound the second-order terms. Doing so yields the quadratic upper bound:
\begin{align} \label{eq:pproof}
%
J(Q_{t+1}) &\leq   J(Q_t) + \langle \nabla J(Q_t) , Q_{t+1} - Q_t \rangle_\ccalH 
\nonumber \\
 &\qquad + \frac{L_Q}{2} \| Q_{t+1} - Q_t \|_\ccalH^2 \; .
%
\end{align}
%
Substitute the fact that the difference between consecutive action-value functions is the projected quasi-stochastic gradient $Q_{t+1} - Q_t  = -\alpha_t \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t')$ \eqref{eq:qprojectedupdateproof} into \eqref{eq:pproof} . 
%
\begin{align} \label{eq:paroof}
%
J(Q_{t+1}) \leq  & J(Q_t) - \alpha_t \langle \nabla J(Q_t) , \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t')\rangle_\ccalH 
\nonumber \\ 
& + \frac{L_Q \alpha_t^2}{2} \| \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') \|_\ccalH^2 \; .
%
\end{align}
%
Subsequently, we use the short-hand notation $\hat{\nabla}_Q J(Q_t):=\hat{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') $ and $\tilde{\nabla}_Q J(Q_t):=\tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') $ for the stochastic and projected stochastic quasi-gradients, \eqref{eq:unprojectedgradproof} and \eqref{eq:projectedgradproof}, respectively. Now add and subtract the inner-product of the functional gradient of $J$ with the stochastic gradient, scaled by the step-size $ \alpha_t \langle \nabla J(Q_t) , \hat{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t') \rangle_\ccalH $, as well as $\alpha_t \|\nabla_Q J(Q_t)\|^2$ into above expression and gather like terms.
%
\begin{align} \label{eq:pbroof}
%
\!\!\!\!\!\!J(\!Q_{t+1}\!)\! &\! \leq   \! J(\!Q_t\!)\!-\! \alpha_t \|\!\nabla_{\!\!Q} J(Q)\|^2\! \!+\! \frac{L_Q \alpha_t^2}{2} \!\| \!\tilde{\nabla}_{\!\!Q} J(Q_t) \!\|_\ccalH^2 \!\!\!
\\ 
&\quad -\! \alpha_t\! \langle \nabla \!J(Q_t\!) , 
\!\!\tilde{\nabla\!\!}_Q J(\!Q_t\!) \!-\!\! \hat{\nabla}_Q J(Q_t\!) \rangle_\ccalH
\nonumber \\
&\quad+ \alpha_t   \langle \nabla J(Q_t) ,
\nabla J(Q_t)- \hat{\nabla}_Q J(Q_t) \rangle_\ccalH  \; 
\nonumber
%
\end{align}
%
Observe that the last two terms on the right-hand side of \eqref{eq:pbroof} are terms associated with the directional error between the true gradient and the stochastic quasi-gradient, as well as the stochastic quasi-gradient with respect to the projected stochastic quasi-gradient. The former term may be addressed through the error bound derived from the KOMP stopping criterion in Proposition \ref{prop_proj_grad_err}, whereas the later may be analyzed through judicious use of the Law of Total Expectation and Assumptions \ref{as:mean_variance_delta} - \ref{as:mean_variance_q}. 

Let's proceed to address the second term on the right-hand side of \eqref{eq:pbroof}. Begin by applying Cauchy-Schwarz to write
\begin{align} \label{eq:qproof}
%
|-\alpha_t\! & \langle \nabla \!J(Q_t\!) , 
\!\!\tilde{\nabla\!\!}_Q J(\!Q_t\!) \!-\!\! \hat{\nabla}_Q J(Q_t\!) \rangle_\ccalH| 
\nonumber \\ 
& \leq \alpha_t \|  \nabla \!J(Q_t\!) \|_\ccalH  \| \tilde{\nabla\!\!}_Q J(\!Q_t\!) \!-\!\! \hat{\nabla}_Q J(Q_t\!) \|_\ccalH 
%
\end{align}
%
Now, apply Proposition \ref{prop_proj_grad_err} to $\| \tilde{\nabla\!\!}_Q J(\!Q_t\!) \!-\!\! \hat{\nabla}_Q J(Q_t\!) \|_\ccalH $, the Hilbert-norm error induced by sparse projections on the right-hand side of \eqref{eq:qproof} and cancel the redundant factor of $\alpha_t$:
%
\begin{align} \label{eq:rproof}
%
\alpha_t\!  \langle \nabla \!J(Q_t\!) , 
\!\!\tilde{\nabla\!\!}_Q J(\!Q_t\!) \!-\!\! \hat{\nabla}_Q J(Q_t\!) \rangle_\ccalH  \leq \epsilon_t \|  \nabla \!J(Q_t\!) \|_\ccalH 
%
\end{align}
%
Next, let's address the last term on the right-hand side of \eqref{eq:pbroof}. To do so, we will exploit Assumptions \ref{as:mean_variance_delta} - \ref{as:mean_variance_q} and the Law of Total Expectation. First, consider the expectation of this term, ignoring the multiplicative step-size factor, while applying \eqref{eq:finitevariance1proof}:
%
\begin{align}\label{eq:total_expectations_1}
%
& \mathbb{E}\big[ \nabla J(Q_t) ,
\nabla_Q J(Q_t)- \hat{\nabla}_Q J(Q_t\!) \rangle_\ccalH\given \ccalF_t \big] \\
&\!\!\!=\!\!\Big\langle\!\!\nabla_{\!\!\!Q} J(Q_t), \mathbb{E} \lbrack  (\!\gamma \kappa(\!(\!\mathbf{s}_t',\mathbf{a}_t'),\!\cdot\!)\! - \!\kappa(\!(\!\mathbf{s}_t,\mathbf{a}_t\!)\!,\!\cdot\!)\!)\!(\!\bar{\delta}_t  \!-\! z_{t+1}\! )\!\given\! \ccalF_t \rbrack \!\!\Big\rangle_{\!\!\!\ccalH} \nonumber
%
\end{align}
%
In \eqref{eq:total_expectations_1}, we pull the expectation inside the inner-product, using the fact that $\nabla_Q J(Q)$ is deterministic. Note on the right-hand side of \eqref{eq:total_expectations_1}, by using \eqref{eq:finitevariance1proof}, we have $\bar{\delta}_t$ inside the expectation in the above expression rather than a realization $\delta_t$.
%
Now, apply Cauchy-Schwartz to the above expression to obtain
%
\begin{align}\label{eq:total_expectations_2}
%
&\Big\langle\!\!\nabla_{\!\!\!Q} J(Q_t), \mathbb{E} \lbrack  (\!\gamma \kappa(\!(\!\mathbf{s}_t',\mathbf{a}_t'),\!\cdot\!)\! - \!\kappa(\!(\!\mathbf{s}_t,\mathbf{a}_t\!)\!,\!\cdot\!)\!)\!(\!\bar{\delta}_t  \!-\! z_{t+1}\! )\!\given\! \ccalF_t \rbrack \!\!\Big\rangle_{\!\!\!\ccalH} \nonumber \\
%
&\leq \|\!\nabla_{\!\!\!Q} J(Q_t\!)\!\|_{\ccalH} \mathbb{E} \lbrack  \|(\!\gamma \kappa(\!(\!\mathbf{s}_t',\mathbf{a}_t'),\!\cdot\!)\!\! - \!\kappa(\!(\!\mathbf{s}_t,\mathbf{a}_t\!)\!,\!\cdot\!)\!)\|_{\ccalH} \nonumber \\
&\quad \times |\!\bar{\delta}_t  \!-\! z_{t+1}\! |\given\! \ccalF_t \rbrack 
%
\end{align}
%
From here, apply the inequality $ab \leq \frac{\rho}{2} a^2  + \frac{1}{2\rho} b^2$ for $\rho>0$ with  $a = |\bar{\delta_t} - z_{t+1}|$, and $b=\alpha_t \| \nabla_Q J(Q_t) \|  \| \gamma \kappa((\mathbf{s}_t',\mathbf{a}_t'),\cdot) - \kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot)\|_\ccalH$, and $\rho=\beta_t$ to the preceding expression:
%
\begin{align}\label{eq:apply_tricky_inequality}
%
\!\!\|\!&\nabla_{\!\!\!Q} J(Q_t\!)\!\|_{\!\ccalH} \mathbb{E} \lbrack  \!\|\!(\!\gamma \kappa(\!(\!\mathbf{s}_t',\!\mathbf{a}_t')\!,\!\cdot\!)\!\! - \!\kappa(\!(\!\mathbf{s}_t,\!\mathbf{a}_t\!)\!,\!\cdot\!)\!)\!\|_{\ccalH}
%
\! |\!\bar{\delta}_t  \!-\! z_{t+1}\! |\!\! \given\!\! \ccalF_t \rbrack \!\!\Big\rangle_{\!\!\!\ccalH} \nonumber \\
%
&\leq \frac{\beta_t}{2} \mathbb{E} \lbrack ( \bar{\delta_t} - z_{t+1} )^2 \mid \mathcal{F}_t \rbrack  \nonumber \\
&+\! \frac{\alpha_t^2}{2 \beta_t}\! \|\!\nabla J(Q_t)\! \|^2_\ccalH \! \mathbb{E}[\| \gamma \kappa(\!(\!\mathbf{s}_t',\mathbf{a}_t'),\cdot\!)\! -\! \kappa((\mathbf{s}_t,\mathbf{a}_t),\cdot)\|_\ccalH^2\given \ccalF_t]
%
\end{align}
%
To \eqref{eq:apply_tricky_inequality}, let's apply Assumption \ref{as:mean_variance_q} regarding the finite second conditional of the difference of reproducing kernel maps \eqref{eq:finitevariance2proof} to the second term, which when substituted into the right-hand side of the expectation of \eqref{eq:pbroof} conditional on $\ccalF_t$, yields
%
%
\begin{align}\label{eq:lemma_iii_near_final}
%
\mathbb{E}[J(\!Q_{t+1}\!)\given\ccalF_t] &\leq   J(\!Q_t\!)
- \alpha_t \!\!\left(\!\!1\! -\! \frac{\alpha_t G_{Q}^2 }{ \beta_t}\!\!\right) \|\nabla_Q J(Q)\|^2\! \!
\nonumber \\ 
&\quad+\!  \frac{\beta_t}{2} \mathbb{E} \lbrack ( \bar{\delta_t} - z_{t+1} )^2 \mid \mathcal{F}_t \rbrack+\frac{L_Q \sigma_Q^2 \alpha_t^2}{2} \nonumber \\
&\quad + \eps_t \|\nabla_Q J(Q_t) \|_{\ccalH} \; ,
%
\end{align}
%
where we have also applied the fact that the projected stochastic quasi-gradient has finite conditional variance \eqref{eq:finitemomentproof} and gathered like terms to conclude \eqref{eq:lemma1iiiproof}. 

\end{myproof}

Lemma \ref{main_lemma} is may be seen as a nonparametric extension of Lemma 2 and A.1 of \cite{wang2017stochastic}, or an extension of Lemma 6 in \cite{pkgtd} to the non-convex case. Now, we may use Lemma \ref{main_lemma} to connect the function sequence generated by Algorithm \ref{qlearning} to a special type of stochastic process called a coupled supermartingale, and therefore prove that $Q_t$ converges to a stationary point of the Bellman error with probability $1$. To the best of our knowledge, this is a one of a kind result.

\begin{lemma}\label{lemma_coupled_supermartingale}
(Coupled Supermartingale Theorem) \cite{bertsekas2004stochastic,wang2017stochastic}. Let $\lbrace \xi_tt\rbrace$, $\lbrace \zeta_t \rbrace$, $\lbrace u_t \rbrace$, $\lbrace \bar{u}_t \rbrace$, $\lbrace \eta_t \rbrace$, $\lbrace \theta_t \rbrace$, $\lbrace \epsilon_t \rbrace$, $\lbrace \mu_t \rbrace$, $\lbrace \nu_t \rbrace$ be sequences of  nonnegative random variables such that
%
\begin{align} \label{eq:zbproof}
%
&\mathbb{E} \lbrace \xi_{t+1} \mid G_t \rbrace \leq (1+\eta_t)\xi_t - u_t + c\theta_t\zeta_t + \mu_t \;,
\nonumber \\ 
&\mathbb{E} \lbrace \zeta_{t+1} \mid G_t \rbrace \leq (1-\theta_t)\zeta_t - \bar{u}_t + \epsilon_t\xi_t + \nu_t
%
\end{align}
%
where $G_t = \lbrace \xi_s, \xi_s, u_s,\bar{u}_s, \eta_s, \theta_s, \epsilon_s, \mu_s, \nu_s \rbrace_{s=0}^t$ is the filtration  and $c > 0$ is a scalar. Suppose the following summability conditions hold almost surely:
%
\begin{align} \label{eq:zcproof}
%
\sum_{t=0}^\infty \eta_t < \infty
\;,
\sum_{t=0}^\infty \epsilon_t < \infty
\;,
\sum_{t=0}^\infty \mu_t < \infty
\;,
\sum_{t=0}^\infty \nu_t < \infty
%
\end{align}
%
Then $\xi_t$ and $\zeta_t$ converge almost surely to two respective nonnegative random variables, and we may conclude that almost surely
%
\begin{equation} \label{eq:zdproof}
%
\sum_{t=0}^\infty u_t < \infty
\;,
\sum_{t=0}^\infty \bar{u}_t < \infty
\;,
\sum_{t=0}^\infty \theta_t \zeta_t < \infty
%
\end{equation}
%
\end{lemma}
%We can use Lemma 2 to establish convergence with probability 1 of Algorithm 1 by considering the expressions derived in Lemma 1.
% \end{myproof} 
\begin{theorem}\label{main_theorem}
Consider the sequence $z_t$ and $\lbrace Q_t\rbrace$ as stated in Algorithm \ref{qlearning}. Assume the regularizer is positive $\lambda > 0$, Assumptions \ref{as:compact}-\ref{as:mean_variance_q} hold, and the step-size conditions hold, with $C>0$ a positive constant:\vspace{-1.5mm}
%
\begin{align} \label{eq:theorem1proof}
%
\sum_{t=1}^\infty \alpha_t  = \infty, \sum_{t=1}^\infty \beta_t  = \infty, \sum_{t=1}^\infty \alpha_t^2 + \beta_t^2 + \frac{\alpha_t^2}{\beta_t}  < \infty , \epsilon_t = C \alpha_t^2 
%
\end{align}
%
Then $ \|\nabla_Q J(Q) \|_{\ccalH}$ converges to null with probability 1, and hence $Q_t$ attains a stationary point of \eqref{eq:lossprob}. In particular, the limit of $Q_t$ achieves the regularized  Bellman fixed point restricted to the RKHS.  
\end{theorem}

 \begin{myproof} \textit{Theorem \ref{main_theorem}}
We use the relations established in Lemma \ref{main_lemma} to construct a coupled supermatingale of the form \ref{lemma_coupled_supermartingale}. First, we use Lemma \ref{main_lemma}\eqref{main_lemma_2}\eqref{eq:lemma1iiproof} to provide an upper bound on Lemma \ref{main_lemma}\eqref{main_lemma_3} \eqref{eq:lemma1iiiproof}.
%
\begin{align} \label{eq:zeproof}
%
\mathbb{E} [J  (\!Q_{t+1}\!) &\given  \ccalF_t] \leq  J(\!Q_t\!)
- \alpha_t \!\!\left(\!\!1\! -\! \frac{\alpha_t G_{Q}^2 }{ \beta_t}\!\!\right) \|\nabla_Q J(Q_t)\|^2\! \!
\nonumber \\ 
+ \!  \frac{\beta_t}{2} (&(1-\beta_t)(z_t - \bar{\delta}_{t-1})^2   + \frac{L_Q}{\beta_t} \|Q_t - Q_{t-1} \|_\ccalH^2 
\nonumber \\ 
&+ \! 2 \beta_t^2 \sigma_\delta^2) \!+ \! \frac{L_Q \sigma_Q^2 \alpha_t^2}{2} + \eps_t \|\!\nabla_{\!Q} J(Q_t) \|_{\ccalH} 
%
\end{align}
%
We introduce three restrictions on the learning rate, expectation rate, and parsimony constant in order to simplify \eqref{eq:zeproof}. First, we assume that $\beta_t \in (0,1)$ for all $t$. Next, we choose $\epsilon_t = \alpha_t^2$. Lastly, we restrict $1 - \frac{\alpha_t G_{Q}^2 }{ \beta_t}  > 0 $, which results in the condition: $\frac{\alpha_t  }{ \beta_t} < \frac{1}{G_{Q}^2}$. Then, we simplify and group terms of \eqref{eq:zeproof}.
%
\begin{align} \label{eq:zfproof}
%
\mathbb{E}[J(\!Q_{t+1}\!)\given  \ccalF_t] \leq &   J(\!Q_t\!)
- \alpha_t \|\nabla_Q J(Q_t)\|^2\! \!
 \\ 
&+ \!  \frac{\beta_t}{2}(z_t - \bar{\delta}_{t-1})^2   + \frac{L_Q}{2} \|Q_t - Q_{t-1} \|_\ccalH^2 
\nonumber \\ 
&+ \beta^3_t \sigma_\delta^2 + \alpha_t^2 \left( \!\!\! \frac{L_Q \sigma_Q^2 }{2} +  \|\nabla_Q J(Q_t) \|_{\ccalH}\! \!\!\!\right) \;
\nonumber
%
\end{align}
%
Next, we aim to connect the result of \eqref{eq:zeproof} to the form of Lemma \ref{lemma_coupled_supermartingale} via the identifications:
%
\begin{align} \label{eq:zgproof}
%
&\xi_t  = J(Q_{t}) \;,  
\zeta_t  = (z_t - \bar{\delta}_{t-1})^2 \;, \theta_t = \beta_t\;, c = 1/2
\\ \nonumber
& u_t = \alpha_t \|\nabla_Q J(Q_t)\|^2\! \! \;, \eta_t  = 0  
\\ \nonumber
& \mu_t \! = \!\! \frac{L_Q}{2} \|Q_t \!\! - \! Q_{t\!-\!1} \|_\ccalH^2 \!\! + \! \beta^3_t \! \sigma_\delta^2 \! + \! \alpha_t^2\! \!\!\left( \!\!\! \frac{L_Q \sigma_Q^2 }{2} \!\!+\!  \|\nabla_{\!Q} J(Q_t) \|_{\ccalH}\!\!\! \right) 
%
\end{align}
%
Observe that $\sum \mu_t < \infty$ due to the upper bound on $\|Q_t \!\! - \! Q_{t\!-\!1} \|_\ccalH^2$ provided by Lemma \ref{main_lemma}\eqref{eq:lemma1iproof} and the summability conditions for $\alpha_t^2$ and $\beta_t^2$ \eqref{eq:theorem1proof}.  

Next, we turn our attention to identifying terms in Lemma  \ref{main_lemma} \eqref{main_lemma_2} \eqref{eq:lemma1iiproof} according to Lemma \ref{lemma_coupled_supermartingale} in addition to \eqref{eq:zgproof}.
%
\begin{align} \label{eq:zhproof}
%
\nu_t = \frac{L_Q}{\beta_t} \|Q_t \! - \! Q_{t-1} \|_\ccalH^2 \! + \! 2 \beta^2_t \sigma_\delta^2  \;, \epsilon_t = 0 \;, \bar{u}_t = 0
%
\end{align}
%
The summability of $\nu_t$ can be shown as follows: the expression $\| Q_t - Q_{t-1}\|^2_\ccalH / \beta_t$ which is order $\mathcal{O}(\alpha_t^2/\beta_t)$ in conditional expectation by Lemma  \ref{main_lemma}\eqref{main_lemma_1}. Sum the resulting conditional expectation for all $t$, which by the summability of the sequence $\sum_t \alpha_t^2 / \beta_t < \infty$ is finite. Therefore, $\sum_t \| Q_t - Q_{t-1}\|^2_\ccalH / \beta_t < \infty$ almost surely.  We also require $\sum_t \beta_t^2 < \infty$ \eqref{eq:theorem1proof} for the summability of the second term of \eqref{eq:zhproof}

Together with the conditions on the step-size sequences $\alpha_t$ and $\beta_t$, the summability conditions of Lemma \ref{lemma_coupled_supermartingale} are satisfied, which allows to conclude that $\xi_t = J(Q_{t}) $ and $\zeta_t = (z_t - \bar{\delta}_{t-1})^2$ converge to two nonnegative random variables w.p. 1, and that
%
\begin{align} \label{eq:zjproof}
%
\!\!\sum_t \!\alpha_t \|\nabla_Q J(Q_t)\|^2 < \infty ,\quad  \sum_t \beta_t (z_t - \bar{\delta}_{t-1})^2 < \infty \;
%
\end{align}
almost surely. Then, the summability of $u_t$ taken together with non-summability of $\alpha_t$ and $\beta_t$ \eqref{eq:theorem1proof} indicates that the limit infimum of the norm of the gradient of the cost goes to null. 
%
\begin{align} \label{eq:zkproof}
%
\liminf_{t \rightarrow \infty} \|\nabla_Q J(Q_t) \| = 0 \;, 
\liminf_{t \rightarrow \infty} (z_t - \bar{\delta}_{t-1})^2 = 0 
%
\end{align}
%
almost surely. 
From here, given $\liminf_{t \rightarrow \infty} \|\nabla_Q J(Q_t) \|_{\ccalH} = 0$, we can apply almost the exact same argument by contradiction as \cite{wang2017stochastic} to conclude that the whole sequence $\|\nabla_Q J(Q_t) \|_{\ccalH}$ converges to null with probability $1$, which is repeated here for completeness.

 Consider some $\eta>0$ and observe that $\|\nabla_Q J(Q_t)\|_{\ccalH}\leq \eta$ for infinitely many $t$. Otherwise, there exists $t_0$ such that $\sum_{t=0}^\infty \|\alpha_t\nabla_Q  J(Q_t)\|_{\ccalH}^2 \geq \sum_{t=t_0}^\infty \alpha_t \eta^2 =\infty$ which contradicts \eqref{eq:zjproof}. Therefore, there exists a closed set $\bar{\ccalH} \subset \ccalH$ such that $\{Q_t\}$ visits $\bar{\ccalH}$ infinitely often, and
 %
 \begin{align}\label{eq:cases_functional_gradient1}
 \|\nabla_Q J(Q) \|_{\ccalH} 
 \begin{cases} 
 \leq \eta \text{ for } Q\in\bar{\ccalH} \\
 > \eta \text{ for  } Q \not\in\bar{\ccalH}, Q \in \{Q_t \}
 \end{cases}
 \end{align}
%
Suppose to the contrary that there exists a limit point $\tilde{Q}$ such that $\|\nabla_Q J(\tilde{Q})\|_{\ccalH} > 2 \eta$. Then there exists a closed set $\tilde{\ccalH}$, i.e., a union of neighborhoods of all $Q_t$'s {such that $\|\nabla_Q J(Q_t)\|_{\ccalH} > 2 \eta$, with $\{Q_t\}$ visiting $\tilde{\ccalH}$ infinitely often}, and 
%
 \begin{align}\label{eq:cases_functional_gradient2}
 \|\nabla_Q J(Q) \|_{\ccalH} 
 \begin{cases} 
 \geq 2\eta \text{ for } Q\in\tilde{\ccalH} \\
 < 2\eta \text{ for  } Q \not\in\tilde{\ccalH}, Q \in \{Q_t \}
 \end{cases}
 \end{align}
%
Using the continuity of $\nabla J$ and $\eta>0$, we have that $\bar{\ccalH}$ and $\tilde{\ccalH}$ are disjoint: $\text{dist}(\bar{\ccalH},\tilde{\ccalH}) > 0$. Since $\{Q_t\}$ enters both $\bar{\ccalH}$ and $\tilde{\ccalH}$ infinitely often, there exists a subsequence {$\{Q_t\}_{t\in\ccalT} = \{ \{Q_t\}_{t=k_i}^{j_i-1}\}$} (with $\ccalT \subset \mathbb{Z}^+$) that enters  $\bar{\ccalH}$ and $\tilde{\ccalH}$ infinitely often, with $Q_{k_i} \in  \bar{\ccalH}$ and $Q_{j_i}\in \tilde{\ccalH}$ for all $i$. Therefore, for all $i$, we have
%
\begin{align}\label{eq:grad_inequality_eta}
&\|\nabla_Q J(Q_{k_i}) \|_{\ccalH} \geq 2 \eta> \|\nabla_Q J(Q_{t}) \|_{\ccalH}    \\
&> \eta \geq \|\nabla_Q J(Q_{j_i}) \|_{\ccalH} \quad\text{ for } t = k_i +1 , \dots, j_i -1\nonumber
\end{align}
%
Therefore, we can write 
%
\begin{align}\label{eq:divergence_setdist}
%
\sum_{t\in\ccalT} \|Q_{t+1} - Q_t \|_{\ccalH} &=\sum_{i=1}^\infty \sum_{t={k_i}}^{j_i-1} \|Q_{t+1} - Q_t \|_{\ccalH}  \\
&\hspace{-3mm}\geq \sum_{i=1}^\infty \|Q_{k_i} - Q_{j_i} \|_{\ccalH} \geq \text{dist}(\bar{\ccalH},\tilde{\ccalH}) = \infty\nonumber
%
\end{align}
%
However, we may also write that 
%
\begin{align}\label{eq:convergence_gradient}
%
\infty> \sum_{t=0}^\infty \alpha_t \|\nabla J(Q_t) \|_{\ccalH}^2 \geq \sum_{t\in\ccalT} \alpha_t \|\nabla J(Q_t) \|_{\ccalH}^2 > \eta^2 \sum_{t\in\ccalT} \alpha_t 
%
\end{align}
Then, using the fact that the sets $\ccalX$ and $\ccalA$ are compact, there exist some $M>0$ such that $\|Q_{t+1} - Q_t \|_{\ccalH}\leq \alpha_t \| \tilde{\nabla}_Q J(Q_t, z_{t+1}; \mathbf{s}_t,\mathbf{a}_t,\mathbf{s}_t')\|_{\ccalH} \leq M \alpha_t$ for all $t$, using the fact that $\eps_t = \alpha_t^2$. Therefore, 
%
\begin{align}\label{eq:divergence_setdist}
%
\sum_{t\in\ccalT} \|Q_{t+1} - Q_t \|_{\ccalH} \leq M \sum_{t\in\ccalT} \alpha_t <\infty
%
\end{align}
which contradicts \eqref{eq:divergence_setdist}. Therefore, there does not exist any limit point $\tilde{Q}$ such that $\|\nabla_Q J(\tilde{Q}) \|_{\ccalH} > 2 \eta$. By making $\eta$ arbitrarily small, it means that there does not exist any limit point that is nonstationary. Moreover, we note that the set of such sample paths occurs with probability $1$, since the preceding analysis applies to all sample paths which satisfy \eqref{eq:zjproof}. Thus, any limit point of $Q_t$ is a stationary point of $J(Q)$ almost surely.
%
\end{myproof}

Theorem \ref{main_theorem} establishes that Algorithm \ref{qlearning} converges almost surely to a stationary solution of the problem \eqref{eq:lossprob} defined by the Bellman optimality equation in a continuous MDP. This is one of the first Lyapunov stability results for $Q$-learning in continuous state-action spaces with nonlinear function parameterizations, which are intrinsically necessary when the $Q$-function does not admit a lookup table (matrix) representation, and should form the foundation for value-function based reinforcement learning in continuous spaces. A key feature of this result is that the complexity of the function parameterization will not grow untenably large due to the use of our KOMP-based compression method which ties the sparsification bias $\eps_t$ to the algorithm step-size $\alpha_t$. In the following section, we investigate the empirical validity of the proposed approach on a classic autonomous control task called the Continuous Mountain Car.

==> softmax.tex <==


To handle the maximization of a finite number of variables, we can use the softmax 
%
\begin{align}  \label{eq:soft1} 
%
f(x) = \log(e^{x_1} + \ldots +e^{x_m} )
%
\end{align}
%
This is a good idea because we know that:
%
\begin{align}  \label{eq:soft2} 
%
\max(x_1, \ldots, x_m) \leq f(x) \leq max(x_1, \ldots, x_m) + \log m
%
\end{align}
%
So, we are within $\log m$ of the actual maximum. Instead, we can use:
%
\begin{align}  \label{eq:soft3} 
%
f_\alpha(x) = \frac{1}{\alpha}log(e^{\alpha x_1} + \ldots +e^{\alpha x_m} )
%
\end{align}
%
If we use $f_\alpha$ instead of $f$, we have:
%
\begin{align}  \label{eq:soft4} 
%
\frac{1}{\alpha} \max(x_1, \ldots, x_m) \leq f_\alpha(x) \leq \frac{1}{\alpha}max(\alpha x_1, \ldots, \alpha x_m) + \frac{log m}{\alpha}
%
\end{align}
%
Thus, the bound improves by a factor of $\frac{1}{\alpha}$. In particular, for $\alpha$ sufficiently large, the max and the softmax are indistinguishable. In fact:
%
\begin{align}  \label{eq:soft5} 
%
\lim_{\alpha \rightarrow \infty} f_\alpha(x) = \max(x_1, \ldots, x_m)
%
\end{align}
%
In the continuous case, we use the softmax: 
%
\begin{align}  \label{eq:soft6} 
%
g_{\alpha}(Q,s) = \frac{1}{\alpha} \log(\int_a e^{\alpha Q(s,a)}da)
%
\end{align}
%
When we take the functional gradient of $g_\alpha(Q,s)$, we obtain: 
%
\begin{align}  \label{eq:soft7} 
%
\nabla_Q g_{\alpha}(Q,s) = \frac{1}{\alpha} \frac{1}{\int e^{\alpha Q(s,a)}da} \int \alpha e^{\alpha Q(s,a)} \kappa((s,a),\cdot) da
%
\end{align}
%
Thus, the derivative is a ratio of two integrals:
%
\begin{align}  \label{eq:soft8} 
%
\nabla_Q g_{\alpha}(Q,s) = \frac{\int e^{\alpha Q(s,a)} \kappa((s,a), \cdot) da}{\int e^{\alpha Q(s,a)}da} 
%
\end{align}
%
Now, we can examine the case where $\alpha$ is large:
%
\begin{align}  \label{eq:soft9} 
%
a' := \arg \max_a Q(s,a)
%
\end{align}
%
and observe that as $\alpha$ grows, the mass concentrates around $a'$. The gradient can be approximated as:
%
\begin{align}  \label{eq:soft9} 
%
\hat{\nabla}_Q g_{\alpha}(Q,s) =  \frac{ e^{\alpha Q(s,a)} \kappa((s,a), \cdot) }{ e^{\alpha Q(s,a)}}  = \kappa((s,a), \cdot)
%
\end{align}
%

